See More and Know More: Zero-shot Point Cloud Segmentation via Multi-modal Visual Data

Zero-shot point cloud segmentation aims to make deep models capable of recognizing novel objects in point cloud that are unseen in the training phase. Recent trends favor the pipeline which transfers knowledge from seen classes with labels to unseen classes without labels. They typically align visual features with semantic features obtained from word embedding by the supervision of seen classes' annotations. However, point cloud contains limited information to fully match with semantic features. In fact, the rich appearance information of images is a natural complement to the textureless point cloud, which is not well explored in previous literature. Motivated by this, we propose a novel multi-modal zero-shot learning method to better utilize the complementary information of point clouds and images for more accurate visual-semantic alignment. Extensive experiments are performed in two popular benchmarks, i.e., SemanticKITTI and nuScenes, and our method outperforms current SOTA methods with 52% and 49% improvement on average for unseen class mIoU, respectively.

==> sections/5_CLIP.tex <==
\begin{table}[t]
\begin{center}
\caption{CLIP model experiment on SemanticKITTI dataset with the 4-unseen-class setting.}
% \vspace{-1ex}
\label{table:clip_model}
\resizebox{\linewidth}{!}{
\begin{tabular}{lcccc}
\toprule
\multirow{2}{*}{Model}       & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Seen\\ mIoU\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Unseen\\ mIoU\end{tabular}} & \multicolumn{2}{c}{Overall}   \\ \cline{4-5}  & & & \multicolumn{1}{c}{mIoU} & \multicolumn{1}{c}{hIoU} \\ \midrule
%TGP + CLIP text encoder & 56.3 & 9.0 & 46.3 & 15.5  \\
%TGP\cite{chen2022zeroshot}   & 54.6 & \textbf{17.3} & \textbf{46.7} & \textbf{26.3}\\ \hline
Ours $\leftarrow$ CLIP model   & 56.6 & 14.1 & 47.7 & 22.6          \\
Ours     & \textbf{58.8} & \textbf{26.8} & \textbf{52.1} & \textbf{36.8}  \\ \bottomrule
\end{tabular}
}
\end{center}
% \vspace{-5ex}
\end{table}

Given the success of the CLIP \cite{CLIP} model in 2D zero-shot segmentation \cite{Xu2021clip1, Lddecke2022clip2, Ding2022Decouplingclip3, Li2022LanguagedrivenSS, zhou2022extract}, we aim to investigate its potential for 3D point cloud semantic segmentation by incorporating the CLIP model into our method. We follow the approach used in MaskCLIP \cite{zhou2022extract}, where the class name is inserted into 85 hand-crafted prompts and they are fed into CLIP's text encoder to generate multiple text features. Additionally, we replace the 2D ResUNet backbone with MaskCLIP+.
As shown in Table \ref{table:clip_model}, even though unseen objects may already occur in the CLIP training data, causing data leakage, the incorporation of the CLIP model still performs worse than our \textbf{pure zero-shot method}.
It is mainly because CLIP is based on the contrastive learning between image and text pairs and the significant disparity between point cloud features and image features makes point cloud visual features difficult to align with semantic features extracted by CLIP. 
However, it is interesting to explore the projection between point cloud and images and transfer the knowledge learnt by CLIP to solve 3D zero-shot problems in large scenarios.
